Towards Massive Interaction with Generalist Robotics: A Systematic Review of XR-enabled Remote Human-Robot Interaction Systems

The rising interest of generalist robots seek to create robots with versatility to handle multiple tasks in a variety of environments, and human will interact with such robots through immersive interfaces. In the context of human-robot interaction (HRI), this survey provides an exhaustive review of the applications of extended reality (XR) technologies in the field of remote HRI. We developed a systematic search strategy based on the PRISMA methodology. From the initial 2,561 articles selected, 100 research papers that met our inclusion criteria were included. We categorized and summarized the domain in detail, delving into XR technologies, including augmented reality (AR), virtual reality (VR), and mixed reality (MR), and their applications in facilitating intuitive and effective remote control and interaction with robotic systems. The survey highlights existing articles on the application of XR technologies, user experience enhancement, and various interaction designs for XR in remote HRI, providing insights into current trends and future directions. We also identified potential gaps and opportunities for future research to improve remote HRI systems through XR technology to guide and inform future XR and robotics research.

==> Chapters/Introduction-old.tex <==
\section{Introduction}

Remote collaboration means the disappearance of distance and can support flexible work and lifestyles that are not bound by geography, even working together across time zones and cultures~\cite{wang2021ar}. With the development of communication and mobile technologies, videoconferences and teleconferences have been widely used as remote collaboration solutions, however, simple video interfaces can face a lack of intuitiveness when solving complex tasks (e.g., maintenance instruction, lab teaching)~\cite{wang2021ar,schafer2021survey}. Augmented reality (AR), virtual reality (VR) and mixed reality (MR) technologies are becoming more sophisticated, and many compact and lightweight devices suitable for remote collaboration are within reach, opening up new avenues for remote collaboration.

We are in the midst of the fourth industrial revolution or Industry 4.0, and Industry 4.0 projects encourage human-robot collaboration, a type of system known as human-robot collaboration (HRC)~\cite{hashemi2020operations,hao2017role,yew2017immersive}. Cyber-Physical Systems (CPS), a component of Industry 4.0, also emphasizes the interaction between humans and machines~\cite{hao2017role}. Robots controlled remotely by humans perform a decisive role in dangerous, unstructured and unrecognized situations and environments. However, human operators are still commonly confronted with the lack of an intuitive control interface due to the lack of proper feedback and complex methods of entering motion commands~\cite{jung2018robotic}. This can lead to less efficient interactions or even to task failure. Also, traditionally, interaction with robots often relies on the internal physical or visual feedback capabilities of the robot, however, this approach makes it difficult to provide expressive physical feedback that extends beyond internal capabilities~\cite{suzuki2022augmented}. Virtual, augmented, and mixed reality (VAM) offer new ways to modulate human-robot interaction, and in recent years, a variety of research has been completed based on VAM to improve the intuitiveness of human-robot remote interfaces~\cite{suzuki2022augmented,malik2020virtual,wang2021ar}. Despite the importance of remote human-robot collaboration in complex systems and manufacturing engineering management, and the natural interaction between humans and computers that VAM can support, VAM-based remote human-robot collaboration remains an under-researched topic.
 
\subsection{VAM-based Remote Collaboration and Human-robot Collaboration}

In recent years, VAM-based real-time and not real-time remote collaboration systems have gained prominence in applications in topics such as healthcare, education, training, and engineering assistance, especially in the wake of the COVID-19 pandemic.~\cite{wang2021ar} Augmented reality (AR) is a technology that enhances the real world by superimposing computer-generated virtual content on the real world through various perceptual information channels (e.g., audio, visual, and haptic).~\cite{lee2021towards} In this paper, we will only discuss immersive virtual reality (VR), such as CAVE technology or VR glasses or other types of head-mounted displays (HMD), virtual reality technology can simulate the real world and make players feel like they are really being there.~\cite{freina2015literature} For the definition of mixed reality (MR), we refer to the definition of the reality-virtual continuum by Speicher et al.~\cite{speicher2019mixed} and describe mixed reality as a region where the real and virtual worlds are mixed. Remote collaboration requires local users to share and perceive collaborative states with remote objects (users or physical entities), express collaborative intent, and manipulate physical or virtual subjects.~\cite{wang2021ar} VAM technology allows us to design visual and even more sensory feedback beyond physical reality, making expression more natural and intuitive. Sharing non-verbal cues such as gestures, annotations, and instructions in remote VAM systems has also been shown to be more efficient and engaging in collaboration.~\cite{gao2016oriented,teo2019investigating,teo2019mixed}

Automation in manufacturing is one of the trends in industry, but for many industries, the implementation of fully automated systems still faces considerable challenges.~\cite{hashemi2020operations} Advances in sensor devices have brought new types of robots that can cooperate with humans and solve a wide variety of tasks - collaborative robots that interact directly with humans in a defined collaborative workspace.~\cite{hashemi2020operations,vysocky2016human,shu2018human} These robots also introduce the concept of human-robot collaborative systems. Robots have the speed, precision, tirelessness, and power to replace laborers performing non-ergonomic tasks.~\cite{hashemi2020operations,vysocky2016human} However, robots do not have the ability to think independently and are limited by programming, some unexpected situations or tasks that robots cannot fully replace (such as innovation or design) still require human involvement at this stage as well. In today's society, robots are no longer limited to manufacturing environments, but are also available in families, offices, hospitals, and other more complex human work environments.~\cite{bauer2008human} It is more urgent to strengthen the understanding between human and robot and break the interaction barrier between both.

Effective human-robot cooperation faces multiple challenges, including the generation of intention-expressive motion, interpretable task plans, verbalization of natural language intentions, and explicit signaling mechanisms.~\cite{suzuki2022augmented} While the small displays used by ordinary robots for interaction are unable to present expressive information~\cite{suzuki2022augmented}, VAM provide new ways to modulate human-robot interaction and enable communication. Suzuki et al.'s~\cite{suzuki2022augmented} results suggest that humans prefer robots to present their intentions directly as visual cues. In the last few decades, there has been a increasing amount of work integrating VAM into human-robot collaboration systems, such as AR to help automate robot programming~\cite{bambusek2019combining}, controlling real robots on mobile platforms using augmented reality (AR) technology~\cite{gong2019projection}, using VR for simulation experiments~\cite{dombrowski2017interactive}, and using robot operating systems (ROS) as middleware to drive robots in VR with feedback to users via HMDs~\cite{de2017human}. A virtual reality human-robot collaborative welding system that combines the advantages of human (adaptive intelligence) and robot (higher motion accuracy and physical limitations)~\cite{wang2019virtual}.

Some studies have explored human-robot collaboration in remote work environments, however, these research projects tend to be individual explorations with little systematic analysis of the design space and research questions in VAM-based research on human-robot collaboration in remote environments.

\subsection{Methodology and Previous Survey}

This survey article presents findings from a systematic literature review of human-robot interaction based on VAM technology in remote environments, where we review a sample of works published over a ten-year period from 2012 to 2022, for a total of XXX articles...

We used the PRISMA method described by Page et al.~\cite{page2021prisma} to systematically conduct a literature survey and used the web-based tool Covidence to collaborate with multiple authors to handle this process. We found these articles mainly through publication databases such as ACM Digital Library and IEEE Xplore, and the keywords chosen were the three dimensions of remote, human-robot interaction and VAM technology. Considering the terminological expressions in different contexts, we selected the keywords "distributed", "remote" and "spatial" for the remote environment. The main keywords involved in human-robot interaction are "robotic", "robot", "machine", "human-robot interaction", "human-robot collaboration", "interaction ", "collaboration", "cooperation", "collaborate" and the abbreviations "HRI" and "HRC", the keywords and abbreviations related to VAM technology we have chosen "virtual reality", "virtual reality" and "virtual reality". "augmented reality", "mixed reality", "vr", "ar" and "mr".

VAM technology, remote collaboration, and human-robot interaction have all been subject to various literature surveys or reviews in the past, however the intersection of the three dimensions has not been addressed, especially remote human-robot interaction. Schafer et al.~\cite{schafer2021survey} and Wang et al.~\cite{wang2021ar} reviewed remote collaboration systems based on VAM technology, where Schafer et al. focused more on synchronous remote collaboration systems, while Wang et al. focused on physical tasks. For human-robot interaction systems or collaborative robots, the vast majority of researchers have focused only on the application of AR technology~\cite{suzuki2022augmented,bassyouni2021augmented,makhataeva2020augmented,costa2022augmented,de2020systematic,green2007human,phaijit2022taxonomy}, Dianatfar et al.~\cite{dianatfar2021review} and Bric et al.'s~\cite{bric2016current} survey covered VR technology, but the former only summarized VR for surgical robot simulation and did not cover human-robot collaboration, while the latter was an incomplete work. Some of the findings mentioned remote environments, such as Jung et al.~\cite{jung2018robotic} but none of the articles systematically categorized and summarized them. In contrast our survey includes all VAM technologies and investigates in depth the problem of human-robot collaboration in remote environments, and we no longer limit the application of robots to industrial scenarios, but include more complex human-involved situations such as homes, hospitals, and schools.

\subsection{Scope of the Present Survey}
